Simulations and flavour-scheme studies for Higgs-boson production in association with charm quarks

We present a detailed NLO+PS study of Higgs-boson production in association with charm and bottom quarks, with particular focus on the modelling of the H+c final state. We systematically compare predictions in massive and massless flavour schemes, quantify scale and flavour-scheme uncertainties, and assess the impact of interference and loop-induced contributions. Special emphasis is placed on the Higgs production via charm Yukawa fusion, for which we compare NLO+PS predictions with a NNLO+PS calculation of $c\bar{c}H$ production in the four-flavour scheme at 13.6 TeV. Based on these results, we provide the first practical recommendations for the simulation of $c\bar{c}H$ production in LHC analyses.

==> utils/preamble_scipost.tex <==
%!TEX root = ../thesis.tex
\RequirePackage{fix-cm} % against warnings for \fontsize

%\documentclass[book,11pt,numbers=noenddot,listof=entryprefix,usegeometry,twoside]{scrreprt}

%\documentclass[12pt,twoside]{scrreprt}
%\usepackage[
%  paperwidth=17cm,
%  paperheight=24cm,
%  inner=2.5cm,
%  outer=2.0cm,
%  top=2.5cm,
%  bottom=2.5cm,
%  includeheadfoot
%]{geometry}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{physics} % for \abs, \dd, ...
%\usepackage{siunitx} % for \micro, \SI
\usepackage{slashed}
\usepackage[T1]{fontenc} % load before inputenc
\usepackage[utf8]{inputenc}
\usepackage{mathpazo} %palatino
%\usepackage{newtxtext,newtxmath}
%\usepackage[scaled]{helvet}
\usepackage[english]{babel}
\usepackage{xifthen} % for \ifthenelse, \isempty
\usepackage{xspace} % for \xspace in macros
\usepackage{verbatim} % Add the verbatim package
\usepackage{booktabs}
%\usepackage{mathrsfs}
\usepackage{makecell}
\usepackage{rotating}

%%%% MATRIX
%%%\usepackage{kbordermatrix}
%%%\renewcommand{\kbldelim}{(}
%%%\renewcommand{\kbrdelim}{)}

% FIGURES
\usepackage{graphicx} %[pdftex],graphics
\usepackage{subfig} % conflicts with tocloft
%\let\subfigure\subfloat% compatibility between subfigure and subfig packages
\usepackage[format=plain,labelfont=bf,skip=6pt]{caption}
%\usepackage{capt-of}
%\usepackage{qtree}
%\usepackage{wrapfig} % to wrap text around figure
\usepackage[bottom]{footmisc} % force footnotes below floats
\usepackage[rightcaption]{sidecap}


%%% FIGURES numbering
%\newcounter{myfigure}
%\renewcommand{\thefigure}{\arabic{myfigure}}
%\newcounter{mytable}
%\renewcommand{\thetable}{\arabic{mytable}}
%\usepackage{makeidx} \makeindex
%\makeglossary

% TABLE
\usepackage[table]{xcolor}
\usepackage{multirow}

%%% PDF
\usepackage{pdfpages} % for \includepdf for title page (load after table package)
\usepackage{tikz} % for drawing, load after multirow to avoid conflict

% REFERENCES
\usepackage[square,numbers,sort&compress]{natbib} % more options for citations, e.g. square brackets
\renewcommand{\bibsection}{}
%\setlength{\bibitemsep}{10pt} % bibtex
\setlength{\bibsep}{0.5\baselineskip} % natbib

% METADATA
% \usepackage[hyperfootnotes=false,backref]{hyperref} % for url hyperlinks; load last to prevent problems %,pagebackref=true

%%%% FEYNMAN FIGURES
%%%\usepackage{feynmp}
%%%\DeclareGraphicsRule{*}{mps}{*}{}
%%%\makeatletter
%%%\def\endfmffile{
%%%  \fmfcmd{\p@rcent\space the end.^^J end.^^J endinput;}
%%%  \if@fmfio
%%%    \immediate\closeout\@outfmf
%%%  \fi
%%%  %\ifnum\pdfshellescape=\@ne
%%%  \ifnum\pdfshellescape>\z@
%%%    \immediate\write18{mpost \thefmffile}
%%%  \fi}
%%%\makeatother

%%% TOC % does not work well with the KOMA class (scrreprt)
% % \usepackage[subfigure,titles]{tocloft}
% % \setlength{\cftbeforechapskip}{0.8em}
% % \setlength{\cftbeforechapskip}{0.8em}
% % \setlength{\cftsecindent}{1.6em}
% % \setlength{\cftsecnumwidth}{2.6em}
% % \setlength{\cftsubsecindent}{4.2em}
% % \setlength{\cftsubsecnumwidth}{3.0em}
% % \setlength{\cftsubsubsecindent}{4.5em}
% % \setlength{\cftsubsubsecnumwidth}{4em}


% EQUATIONS SPACING
\AtBeginDocument{%
 \setlength{\belowdisplayskip}{9pt}%
 \setlength{\belowdisplayshortskip}{9pt}%
 \setlength{\abovedisplayskip}{9pt}%
 \setlength{\abovedisplayshortskip}{9pt}%
}

% BOLD MATH in section titles
% https://tex.stackexchange.com/questions/41379/automatically-typeset-math-in-section-headings-in-bold-face
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother


% NUMBERING LEVEL
\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{2}
%\setcounter{lofdepth}{1} 

% FOOTNOTES
%\newcounter{myfootnote}[chapter]
%\renewcommand{\thefootnote}{\themyfootnote}
%\newcommand{\myfootnote}[1]{\stepcounter{myfootnote}\footnote{#1}}

% LISTS (itemize, enumerate) spacing
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0pt,topsep=6pt}
\setitemize{itemsep=0pt,topsep=6pt}
%%%\renewenvironment{itemize}%
%%%  {\begin{list}{$\bullet$}{%
%%%    \setlength{\topsep}{5pt}%
%%%    %\setlength{\botsep}{5pt}%
%%%    \setlength{\partopsep}{2pt}%
%%%    \setlength{\parsep}{0.5\parskip}%
%%%    \setlength{\itemsep}{2pt}%
%%%    \setlength{\leftmargin}{7ex}%
%%%    \setlength{\rightmargin}{3ex}%
%%%  }}{\end{list}}%


\hyphenation{
  thres-hold dom-i-na-ted
  brems-strah-lung
  re-nor-ma-li-za-tion
  re-nor-ma-li-za-tion-scale
  fac-tor-i-za-tion
  fac-tor-i-za-tion-scale
  part-on-show-er
  part-on-ic
  glu-on-fu-sion
  glu-on-glu-on
  charm-tag-ging
  jet-tag-ging
  cat-e-go-ri-sa-tion
  cat-e-go-ries
  cat-e-go-rised
  mul-ti-var-i-ate
  dis-crim-i-na-tor
  cor-re-la-tion
  sys-tem-at-ic
  un-cer-tain-ties
  pa-ram-e-ter
  pa-ram-e-ters
  per-tur-ba-tive
  per-tur-ba-tive-QCD
  con-ver-gen-ce
  sim-u-la-tion
  sim-u-la-tions
  gen-er-a-tor
  gen-er-a-tors
  fluc-tu-a-tions
  hy-po-the-sis
  hy-po-the-ses
  re-quire-ments
  per-for-mance
  in-ter-po-la-tion
  in-te-gra-tion
  ap-prox-i-ma-tion
  un-cer-tain-ty
  Deep-Jet
  Deep-Flavour
  Deep-JET
  Deep-Flavour-CvsL
  CvsL
  Boost-ed-De-ci-sion-Tree
  FXFX
  Mad-Graph
  aMC-at-NLO
  aMC-at-N-L-O
  aMC
  Py-thia
  NLO
  NNLO
  ISR
  FSR
  me-ta-da-ta
  back-ground
  back-grounds
  sig-nal
  un-tag-ged
  mis-tag-ging
  mis-tag-rate
}


